Light-dependent Impedance Spectra and Transient Photoconductivity in a Ruddlesden-Popper 2D Lead-halide Perovskite Revealed by Electrical Scanned Probe Microscopy and Accompanying Theory

Electric force microscopy was used to record the light-dependent impedance spectrum and the probe transient photoconductivity of a film of butylammonium lead iodide, BA$_{2}$PbI$_{4}$, a 2D Ruddlesden--Popper perovskite semiconductor. The impedance spectrum of BA$_{2}$PbI$_{4}$ showed modest changes as the illumination intensity was varied up to 1400 mW/cm$^{2}$, in contrast with the comparatively dramatic changes seen for 3D lead-halide perovskites under similar conditions. BA$_{2}$PbI$_{4}$'s light-induced conductivity had a rise time and decay time of $\sim$ 100 $\mu$s, 10$^{4}$ slower than expected from direct electron-hole recombination and yet 10$^{5}$ faster than the conductivity-recovery times recently observed in 3D lead-halide perovskites and attributed to the relaxation of photogenerated vacancies. What sample properties are probed by electric force microscope measurements remains an open question. A Lagrangian-mechanics treatment of the electric force microscope experiment was recently introduced by Dwyer, Harrell, and Marohn which enabled the calculation of steady-state electric force microscope signals in terms of a complex sample impedance. Here this impedance treatment of the tip-sample interaction is extended, through the introduction of a time-dependent transfer function, to include time-resolved electrical scanned probe measurements. It is shown that the signal in a phase-kick electric force microscope experiment, and therefore also the signal in a time-resolved electrostatic force microscope experiment, can be written explicitly in terms of the sample's time-dependent resistance (i.e., conductivity).

==> Tirmzi201909__2D_perovskite_conductivity_07_TOC.tex <==
%!TEX root = Tirmzi201909__2D_perovskite_conductivity.tex


\begin{tocentry}
\includegraphics[width=3.5in, height = 2in]{TOC-v2.pdf}
%\caption{}
\label{TOC Graphic}
\end{tocentry}

==> file_1.tex <==



==> file_2.tex <==


